An Impulse-formed Navier-Stokes Solver based on Long-range Particle Flow Maps

We present a particle-grid characteristic-mapping framework that extends long-range characteristic mapping from inviscid flows to general Navier-Stokes dynamics with viscosity, body forces, and complex boundaries. Unlike traditional grid-based and vorticity-centered characteristic methods, our method is built on the observation that particle trajectories naturally provide the long-range flow map, enabling geometric quantities and their gradients to be transported in a direct and effective manner. We identify the impulse, the gauge variable of the velocity field, as the primary quantity mapped along characteristics while remaining compatible with standard velocity-based incompressible solvers. Using the 1-form representation of the impulse equation, we derive an integral formulation that decomposes the impulse evolution into a component transported geometrically along the particle flow map and a complementary component generated by viscosity and body forces evaluated through path integrals accumulated along particle trajectories. These components together yield a unified characteristic-mapping solver capable of handling incompressible Navier-Stokes flows with viscosity and body forces while maintaining the accuracy and geometric fidelity of characteristic transport.

==> backup/metho_zhiqi_tem.tex <==
\section{Characteristic Mapping}

From initial time $s$, consider the fluid domain at arbitrary time $t$ as $U_t, t\ge s$.  For arbitrary velocity field family $u_t: U_t \to R^d, t\ge s$,  the characteristic map is defined as a one-parameter family of maps $\mathbf{X}_t: U_t\to U_s$, satisfying
\begin{equation}\label{eq:characteristic_mapping_equation}
\begin{aligned}
        \partial_t \mathbf{X}_t + (\mathbf{u}\cdot \nabla )\mathbf{X}_t &= 0\\
    X_t(x) &= x
\end{aligned}
\end{equation}
\(\mathbf{X}_t: U_t \to U_s\) is called the characteristic map because for any \( \gamma_0 \in U \), \( \gamma(t) = \mathbf{X}_t(\gamma_0) \) represents a characteristic curve associated with the velocity \( \mathbf{u} \).  Characteristic map can be used to solve the advection equation of a scalar field (or 0-form) \cite{} and the advection equation of a 2-form \cite{}, which method is referred to as Characteristic Mapping. Specifically, for the scalar field $\phi(x,t)$, like vorticity in 2D and level-set function, satisfying the advection equation
\begin{equation}\label{eq:scalar_advection}
\begin{aligned}
    (\partial_t+\mathbf{u}\cdot \nabla)\phi &=0\\
    \phi(\mathbf{x},0) &= \phi_0(\mathbf{x}),    
\end{aligned}
\end{equation}
its solution can be represented as 
\begin{equation}\label{eq:scalar_advection_solution}
    \phi(x,t)=\phi(X_t(x),0) 
\end{equation}
or
\begin{equation}\label{eq:scalar_advection_solution2}
    \phi_t = \mathbf{X}_t^*\phi_s
\end{equation}
with the pullback $\mathbf{X}_t^*\phi_s$ of scalar field $\phi_s$  defined as $(\mathbf{X}_t^*\phi_s)(x) = \phi_s(\mathbf{X}_t(x))$.  The characteristic Mapping method uses Eq. \ref{eq:scalar_advection_solution} to calculate the 2D vorticity field and level-set field from the initial condition directly once the characteristic map $X_t$ is traced by Eq. \ref{eq:characteristic_mapping_equation}. For the vorticity 2-form $\omega = \star(\mathbf{\omega}^\flat)$ in 3D and $\mathbf{\omega}_t: U_t \to \mathbb{R}^d$ is the vector form of the vorticity field, satisfying
\begin{equation}\label{eq:scalar_advection_solution}
    (\partial_t + L_u) \omega = 0 
\end{equation}
in the form of the 2-form, or  
\begin{equation}\label{eq:scalar_advection_solution}
    (\partial_t + L_u) \omega = 0 
\end{equation}
represented by vectors, can be solved by characteristic map $\mathbf{X}_t$ as
\begin{equation}\label{eq:scalar_advection_solution}
    \phi(x,t)=\phi(X_t(x),0) 
\end{equation}
or
\begin{equation}\label{eq:scalar_advection_solution2}
    \phi_t = \mathbf{X}_t^*\phi_s
\end{equation}
with the pullback 

在之前的Characteristic Map方法中，无论是2D还是3D，







For fluid domain $U_t$ at arbitrary time $t$, a map function $X $ can be 


For fluid domain $U_{t_1}$ at time $t_1$ and fluid domain $U_{t_2}$ at time $t_2$, a






In fluid simulation, it is often necessary to solve the advection equation associated with a transport velocity field $\mathbf{u} \in U \times \mathbb{R}_+$, where $U \subset \mathbb{R}^d$ represents the computational domain of interest.  For the advection equation of the scalar field, summarized as 

can be calculated using the Characteristic Mapping method, which directly computes the scalar field $\phi(x,t)$ at the current time $t$ from the initial condition by the traced characteristic map \( X_t: U \times \mathbb{R}_+ \to U \)
\begin{equation}\label{eq:scalar_advection_solution}
    \phi(x,t)=\phi(X_t(x),0) 
\end{equation}
The characteristic map $X_t(x)$ is defined as the solution to, and also computed through, the following vector-valued advection equation:
\begin{equation}\label{eq:characteristic_mapping_equation}
\begin{aligned}
        \partial_t \mathbf{X}_t + (\mathbf{u}\cdot \nabla )\mathbf{X}_t &= 0\\
    X_t(x) &= x
\end{aligned}
\end{equation}
It can be verified that under the definition in Eq. \ref{eq:characteristic_mapping_equation}, Eq. \ref{eq:scalar_advection} and Eq. \ref{eq:scalar_advection_solution} are equivalent,  and thus in the Characteristic Mapping method, once $\mathbf{X}_t$ is computed numerically, any scalar field satisfying Eq. \ref{eq:scalar_advection} can be obtained through Eq. \ref{eq:scalar_advection_solution}.  This method is referred to as the Characteristic Mapping method, since for any \( \gamma_0 \in U \), \( \gamma(t) = \mathbf{X}_t(\gamma_0) \) represents a characteristic curve associated with the velocity \( u \).

For the divergence-free velocity field \( \mathbf{u} \), the characteristic map \( X_t \) defined by Eq. \ref{eq:characteristic_mapping_equation} actually describes the diffeomorphic transformations between \( U \) at time 0 and \( U \) at time \( t \), with the velocity of the flow \( \mathbf{u_t} \) serving as its time derivative $\dot X_t$ at each instance \( t \).  With the definition of pullback of scalar field as $(X_t^*\phi_0)(x) = \phi_0(X_t(x))$,  \ref{} can be represented as $\phi_t = X_t^*\phi_0$.  Correspondingly, 







At each instance ��, the time-derivative Φ¤
�� represents the
velocity of the flow

由$\mathbf{u}$作为生成向量成生成的special diffeomorphism , 即$X_t\in Diff(U)$


The Characteristic Mapping (CM) method consists in computing the  of the domain generated by a given velocity field.

为了使得

Equation \ref{}只能对满足\ref{}的scalar field进行求解，对于3D涡量场，由于其advection equation $(\partial_t+\mathbf{u} \cdot \nabla)\omega-(\omega \cdot \nabla)u=0$ 中额外的stretching term $(\omega \cdot \nabla$，涡向量的分量形式无法通过\ref{}进行advection，从而无法通过Characteristic Mapping直接

为了使得Characteristic Mapping方法能够求解3D 涡量场

为了推广该方法，使得Characteristic Mapping能够解决不满足











can be calculated by Characteristic Mapping method, which 通过追踪到的Characteristic Map
$X_t$ 直接从initial condition中计算当前时间的scalar field.  characteristic map $X_t: U\times R_+ \to U$ 被定义为the following vector-valued advection equation的solution:
\begin{equation}
    
\end{equation}




Here, $\phi$ represents an arbitrary scalar field to be advected, which can be a 2D vorticity field or a 2D/3D level-set field. Direct computation of the advection equation poses many challenges, like introducing additional artificial viscosity for the vortex field \cite{} and having extra regularity requirements on the initial level-set field \cite{}. the Characteristic Mapping method 通过定义


To address these issues, the  has been proposed, based on the equivalence of the advection equation expressed as:
\begin{equation}
    \frac{d}{dt} \phi(\mathbf{\gamma}(t),t) = 0
\end{equation}
or equivalently
\begin{equation}
    \phi(\mathbf{\gamma}(t),t) = \phi(\mathbf{\gamma}(0),0)
\end{equation}
where $\gamma(t)$ is the family of characteristic curves related to the velocity field $\mathbf{u}$, which are determined by their initial positions $\gamma_0$
\begin{equation}
    \begin{aligned}
    \frac{d}{dt}\mathbf{\gamma}(t) = \mathbf{u}(\mathbf{\gamma}(t),t)\\        
    \gamma(0) = \gamma_0
    \end{aligned}
\end{equation}
Characteristic Mapping Method 定义了characteristic map $\mathbf{X}_{[t_1,t_2]}$ to track the characteristic curves 

Characteristic Mapping Method 通过演化直接计算$X$, 以追踪 characteristic curves associateed with velocity u， 并利用\autoref{}从初始条件直接计算任意时刻的标量场，以减少直接计算advection equation导致的涡量场的数值误差和levelset的额外的regularity requirement。 
 
 实际上，这里的$X$表示是 diff

 然后pullback

 在3D的场景下，涡不在是一个



\section{Impulse Representation}


\section{Inclusion of Arbitrary Forces}


\section{Particles As Flow Map}


==> backup/method_zhiqi_with_Lie_before.tex <==
\section{Characteristic Mapping}

\subsection{Foundation of Characteristic Mapping}
From initial time $s$, consider the fluid domain at arbitrary time $t$ as $U_t, t\ge s$.  For arbitrary velocity field family $u_t: U_t \to R^d, t\ge s$,  the characteristic map is defined as a one-parameter family of maps $\mathbf{X}_t: U_t\to U_s$, satisfying
\begin{equation}\label{eq:characteristic_mapping_equation}
\begin{aligned}
        \partial_t \mathbf{X}_t + (\mathbf{u}\cdot \nabla )\mathbf{X}_t &= 0\\
    X_t(x) &= x
\end{aligned}
\end{equation}
\(\mathbf{X}_t: U_t \to U_s\) is called the characteristic map because for any \( \gamma_0 \in U \), \( \gamma(t) = \mathbf{X}_t(\gamma_0) \) represents a characteristic curve associated with the velocity \( \mathbf{u} \).  Characteristic map can be used to solve the advection equation of a scalar field (or 0-form) \cite{} and the advection equation of a 2-form \cite{}, which method is called Characteristic Mapping. Specifically, for the scalar field $\phi(x,t)$, like vorticity in 2D and level-set function, satisfying the advection equation
\begin{equation}\label{eq:scalar_advection}
\begin{aligned}
    (\partial_t+\mathbf{u}\cdot \nabla)\phi &=0\\
    \phi(\mathbf{x},0) &= \phi_0(\mathbf{x}),    
\end{aligned}
\end{equation}
its solution can be represented as 
\begin{equation}\label{eq:scalar_advection_solution}
    \phi(x,t)=\phi(X_t(x),0) 
\end{equation}
or
\begin{equation}\label{eq:scalar_advection_solution2}
    \phi_t = \mathbf{X}_t^*\phi_s
\end{equation}
with the pullback $\mathbf{X}_t^*\phi_s$ of scalar field $\phi_s$  defined as $(\mathbf{X}_t^*\phi_s)(x) = \phi_s(\mathbf{X}_t(x))$.  In the Characteristic Mapping method, equation (\ref{eq:scalar_advection_solution}) is used to calculate the 2D vorticity field and level-set field from the initial condition directly once the characteristic map $X_t$ is traced by equation (\ref{eq:characteristic_mapping_equation}). For the vorticity 2-form $\omega = \star(\mathbf{\omega}^\flat)$ in 3D and $\mathbf{\omega}_t: U_t \to \mathbb{R}^d$ is the vector form of the vorticity field, satisfying
\begin{equation}\label{eq:2_form_advection}
    (\partial_t + \mathbf{u}\cdot \nabla) \mathbf{w}-(\mathbf{w}\cdot \nabla)\mathbf{u} = 0 
\end{equation}
in the form of the 2-form, or  
\begin{equation}\label{eq:2_form_vector_advection}
    (\partial_t + L_u) \omega = 0 
\end{equation}
represented by vectors, can be solved by characteristic map $\mathbf{X}_t$ as
\begin{equation}\label{eq:2_form_advection_solution}
    \mathbf{w}(x,t)=(\nabla X_t)^{-\top}\mathbf{w}(X_t(x),0) 
\end{equation}
or
\begin{equation}\label{eq:2_form_vector_advection_solution}
    \omega_t = \mathbf{X}_t^{*} \omega_s
\end{equation}
with the pullback of 2-form $\omega_s$ is calculated as $(\mathbf{X}_t^{*} \omega_s) = \star[(\nabla X_t)^{-\top}\mathbf{w}(X_t(x),0)]^\flat$.  Equation (\ref{eq:2_form_advection_solution}) is used to calculate the 3D vorticity field from the initial condition directly once the characteristic map $X_t$ is traced by equation (\ref{eq:characteristic_mapping_equation})

\subsection{Limitations of the Characteristic Mapping Method }

In the previous Characteristic Mapping method \cite{}, whether in 2D or 3D, solving the incompressible Euler equations 

\begin{equation}\label{eq:Euler_equation}
    \begin{aligned}
        (\partial_t + u \cdot \nabla) u &= -\nabla p, \\
                        \nabla \cdot u &= 0
    \end{aligned}
\end{equation}
requires converting it into the corresponding vorticity form (\ref{eq:2_form_vector_advection}), using characteristic maps $X_t$ to compute the vorticity field based on equation (\ref{eq:scalar_advection_solution}) and (\ref{eq:2_form_vector_advection_solution}), and converting the vorticity back to the velocity field using Biot-Savart law $u = -\nabla^{-1}\nabla \times w$.  The Characteristic Mapping method can not directly apply to the velocity $u$ and the fundamental reason is that the Characteristic Mapping Method can only be used to solve advection equations, while in the Euler equations for velocity, the presence of the pressure term $\nabla p$ makes the equations no longer advection equations for the velocity.

To apply Characteristic Mapping to the velocity form of the incompressible Euler equation, we need to derive a velocity-related advection equation directly from the Euler equation. In the next chapter, we will introduce how to achieve this using the gauge method.

\section{Impulse-Based Representation}

In this section, we first show the transformation of Euler equations to its impulse gauge form according to \cite{} and then show impulse gauge form of the Euler equation can be solved by the Characteristic Mapping method. 

\subsection{Impulse-Guage Form of Euler Equation}
Following \cite{}, based on the idea of the gauge transform, we first define the impulse variable as \( m = u + \nabla \phi \), where \(\phi\) is to be determined, and transform the Euler equation (\ref{}) into its corresponding impulse form:  
\begin{equation}
\begin{aligned}\label{eq:basic_impulse_equation}
    \frac{D\mathbf{m}}{Dt} + (\nabla \mathbf{u})^\mathrm{T} \mathbf{m} - \nabla \left( \frac{D\phi}{Dt} + \frac{1}{2} \|\mathbf{u}\|^2 - p \right) &= 0\\
    \nabla \cdot (m-\nabla \phi)&= 0\\
\end{aligned}
\end{equation}
Since the velocity \( u \) is divergence-free, \( m = u + \nabla \phi \) can be viewed as performing an Helmholtz-Hodge Decomposition on \( m \), where \( u \) is treated as the divergence-free component of \( m \). As \(\phi\) is undetermined and can be freely chosen, it is possible to select \(\phi\) to satisfy the advection equation \(\frac{D\phi}{Dt} + \frac{1}{2} \|\mathbf{u}\|^2 - p = 0\), thereby eliminating the pressure term \( p \) from equation (\ref{eq:basic_impulse_equation}). The velocity can then be directly obtained through the divergence-free projection of the impulse \( u = Pm \), where \( P \) denotes the divergence-free projection operator:
\begin{equation}
\begin{aligned}\label{eq:impulse_equation}
    \frac{D\mathbf{m}}{Dt} + (\nabla \mathbf{u})^\mathrm{T} \mathbf{m} &= 0\\
     u &= P\mathbf{m}\\
\end{aligned}
\end{equation}

The computation of equation (\ref{eq:impulse_equation}) simply involves first solving the advection equation to obtain \( m \), and then applying a projection to derive the velocity \( u \) at each substep. This process is essentially consistent with the approach of directly solving equation (\ref{eq:Euler_equation}) using a time-split framework, namely, solving the advection term \( (u \cdot \nabla)u \), followed by projection to compute the pressure term \( \nabla p \). Unlike the vortex method that the previous Characteristic Mapping approach is based on, which requires using the Biot-Savart law to convert \( \mathbf{w} \) into \( \mathbf{u} \), this method avoids that complexity. Therefore, through the Gauge Transform, we have achieved our initial goal of deriving a velocity-related advection equation that does not include the pressure term.

\subsection{Characteristic Mapping with Impulse-Guage Form}




\section{Particles As Flow Map}

\section{Inclusion of Arbitrary Forces}



==> discussion.tex <==
\section{Discussion}

==> introduction_prev.tex <==
\section{Introduction}
\subsection{Impulse Gauge Variable}
The impulse gauge variable was first introduced as a Lagrangian numerical method by \citep{buttke1992lagrangian}, where impulse was denoted as velicity, and was further explored in \citep{cortez1994approximation, cortez1995impulse}. The impulse is defined as any vector field that differs from the solution $\bm{u}$ of the incompressible Euler's equation by a gradient field \citep{buttke1992lagrangian}. However, as noted by \citep{cortez1995impulse}, the velocity field induced by impulse methods exhibits greater singularity compared to vortex methods because of the additional differentiation introduced the velocity reconstruction process, necessitating the use of a cutoff function to smoothly mitigate these singularities. Additionally, the impulse carried by a particle continuously accumulates \citep{}, leading to numerical instability. 

In this paper, we introduce a hybrid numerical method based on flow map techniques developed in both the CFD \citep{yin2021characteristic, yin2023characteristic} and graphics \citep{zhou2024eulerian} communities, where impulse serves as the primary variable. To ensure numerical stability, our method incorporates periodic re-initialization, akin to how the remeshing techniques are employed in many hybrid vortex methods \citep{koumoutsakos1995high, huberson1990correction}. Furthermore, we extend the definition of the impulse variable to solve the Navier-Stokes equations.

% \subsection{Eulerian-Lagrangian Methods}
% Particle-In-Cell (PIC) methods were originally proposed centuries ago and have since been improved in various ways to address the Navier-Stokes equations, leading to the development of methods such as FLIP, APIC, XPIC, and EPIC. Among these, HOPIC \citep{edwards2012high} introduced the first high-order convergence scheme within the Eulerian-Lagrangian framework, achieving fifth-order accuracy by employing Moving Least Squares (MLS) for particle-to-grid transfers, Weighted Essentially Non-Oscillatory (WENO) schemes for interpolation, and Runge–Kutta methods for temporal discretization in the absence of solid boundaries. However, the simultaneous use of MLS and WENO kernels introduces substantial computational costs, making the method resource-intensive. 

% Subsequent Eulerian-Lagrangian methods have focused on improving the interpolation kernel accuracy, such as in quadratic PolyPIC\citep{}, and adopting MLS kernels for particle-to-grid transfers\citep{}. Recently, a new approach to improving accuracy in Eulerian-Lagrangian schemes was introduced, where flow map quantities are carried with particles (PFM) \citep{}. This approach demonstrated significant improvements in vorticity preservation under Euler’s equation settings and was later extended to handle Navier-Stokes equations in the presence of viscosity \citep{}. However, these methods lack rigorous convergence tests and benchmarking against established schemes.

In this work, we modify the PFM framework to solve the Navier-Stokes equations while avoiding the accumulation of pressure buffers, as proposed in \citep{}, which can introduce additional numerical errors. We thoroughly test the proposed PFM method across various benchmark problems and compare its performance with existing hybrid Eulerian-Lagrangian schemes such as FLIP, APIC, and VIC. Our results indicate that the proposed method achieves improved convergence rates, numerical accuracy, and vorticity preservation compared to these methods. Furthermore, we compare our method with the high-order WENO5 scheme \citep{liu1994weighted} and show that it achieves comparable accuracy while maintaining computational efficiency. Using the original quadratic kernel from APIC for both particle-to-grid transfer and grid interpolation, our approach provides a balance between accuracy and efficiency, making it a promising alternative for fluid dynamics simulations.


==> introduction_zhiqi.tex <==
\section{Introduction}

Developing numerical algorithms to simulate incompressible fluids plays a vital role in various fields across science and engineering. The accuracy of these simulations directly affects the reliability of flow prediction and engineering design. Improving the precision and stability of simulations, particularly by preserving spatiotemporal coherent vortical structures, has long been a central focus in research.

%Traditional methods face challenges in preserving key structures and features of fluid flow. Traditional fluid simulation methods are typically categorized into Eulerian and Lagrangian approaches. Eulerian methods discretize physical quantities on fixed spatial grids, allowing accurate and efficient computation of spatial operators. High-resolution grids can capture fine flow structures, but these methods often struggle with tracking flow characteristics during advection, leading to numerical dissipation and loss of detail, especially in highly deformable flows. Lagrangian methods, on the other hand, track fluid particles that move with the flow, carrying physical quantities along their trajectories. Fluid particles can naturally preserve flow characteristics and handle advection. However, the lack of a structured grid makes spatial derivatives less accurate, and discretization errors can still result in the loss of key flow features.

Traditional methods face challenges in preserving characteristics of fluid flow. Pure Eulerian methods struggle with accurately capturing characteristics in advection, while pure Lagrangian methods suffer from inaccuracies in spatial derivative calculations. Hybrid approaches, such as the semi-Lagrangian method, aim to combine their strengths by computing advection via backward particle and transport Eulerian quantities on the grid. While semi-Lagrangian methods improve characteristic preservation, repeated interpolation in short-step mappings can introduce numerical dissipation.  In recent years, a new class of characteristic mapping methods \cite{nave2010gradient, kolomenskiy2016adaptive, mercier2013characteristic, yin2021characteristic,yin2023characteristic, wang2024eulerian} has been proposed, extending the concept of semi-Lagrangian approaches, offering strong capability in preserving flow characteristics. These methods construct a long-term mapping from the initial time to the current time, enabling fluid characteristics, like vorticity \cite{yin2021characteristic,yin2023characteristic,wang2024eulerian}, to be updated via direct pullback from the initial condition. This approach avoids cumulative interpolation error and allows for non-dissipative simulation of inviscid Euler flows.

For incompressible flow, the characteristic mapping method relies on a vorticity-based formulation of the fluid and requires a framework based on complex fourth-order Hermite interpolation, namely GALS framework \cite{nave2010gradient}, to construct the characteristic map. Moreover, it lacks a mechanism for extension to the Navier-Stokes (NS) equations with viscous force, which limits its broader applicability. In this paper, we explore a velocity-based approach and propose a simpler method for characteristic map construction, based on the idea of using the particles themselves as the characteristic map. Building on this, we introduce a new framework, the Particle Flow Map (PFM), and further develop a technique that enables its extension to more general Navier-Stokes equation simulations.

We aim to explore a velocity-based approach; however, for incompressible fluids, the velocity field cannot naturally follow a characteristic mapping due to the divergence-free constraint, which prevents direct mapping from the initial velocity. The classical impulse method introduced by Buttke \cite{buttke1992lagrangian}, addresses this by introducing a gauge transformation \( \mathbf{m} = \mathbf{u} + \nabla \phi \), where the impulse variable \( \mathbf{m} \) evolves independently of the incompressibility condition and thus supports a characteristic mapping formulation. While prior work \cite{buttke1992lagrangian, buttke1993velicity, buttke1993turbulence, cortez1995impulse, cortez1996impulse, cortez1998accuracy, cortez2000vortex, summers2000representation} focused on evolving \( m \) using Lagrangian methods and largely overlooked its mapping form, we find that this mapping form plays a crucial role in preserving the fluid’s characteristic behavior. In this paper, we treat impulse as the primary variable and evolve it through a long-term characteristic mapping, recovering velocity at each step via a standard incompressibility projection. This results in a characteristic-mapping framework based on the transformed velocity, which circumvents the challenge of reconstructing the harmonic component of the velocity field \cite{mizukami1983stream, tezduyar1988petrov, 10.1145/3592402} in vorticity-based methods. Previous characteristic mapping methods \cite{yin2021characteristic,yin2023characteristic}, derived from the vortex formulation of the Euler equations, are limited to inviscid flows and lack a clear mechanism for extension to the Navier–Stokes (NS) equations, which limitation also applies to impulse-based mapping formulation \cite{buttke1992lagrangian}. To overcome this, we leverage the Lie derivative form of the NS equations in impulse formulation to derive a new path integration scheme, enabling the impulse-based mapping framework to handle viscous flows and serve as a solver for the full NS equations.

Previous characteristic mapping methods constructed the mapping on a grid using Hermite interpolation, which requires complex computation of the gradient information of the characteristic map. In this paper, we propose an alternative and more natural way to construct the characteristic mapping. To distinguish it from the Hermite interpolation-based approach, we refer to it as the flow map method. The flow map method draws inspiration from Eulerian–Lagrangian hybrid particle/grid approaches, which use grids for pressure and viscosity computations while employing particles for advection to minimize numerical diffusion.  This idea first realized in the Particle-in-Cell (PIC) method \cite{harlow1964particle}, which, however, suffered from smoothing errors during particle-to-grid transfers. This limitation was addressed by FLIP \cite{brackbill1986flip}, which updated particle velocities using velocity increments to better preserve vorticity. Subsequent improvements, including APIC \cite{jiang2017angular}, XPIC \cite{hammerquist2017new}, and EPIC \cite{frey2022epic}, introduced higher-order moment transfers, culminating in HOPIC \cite{edwards2012high}, which achieves fifth-order accuracy using MLS, WENO schemes, and Runge–Kutta integration. To retain high accuracy with reduced reliance on complex interpolation kernels, methods such as PolyPIC \cite{fu2017polynomial} and unified MLS-based frameworks \cite{hu2018moving} have also been developed.  Although these methods compute advection using particles, they have not recognized the inherent nature of particles as carriers of long-term characteristic mappings. Instead, they only compute one-step velocity advection and require velocity updates from the grid at each step, resulting in repeated interpolations that still introduce numerical dissipation.  In this paper, we leverage the fact that fluid particles naturally carry long-term characteristic mapping information and, based on the impulse mapping formulation, directly map the initial velocity field to obtain the current impulse field. This results in a non-dissipative computational method similar to characteristic mapping methods, but without the need for complex gradient computations required by Hermite interpolation.


In recent years, impulse-based approaches and the concept of particles as flow maps have gained increasing attention in computer graphics for their enhanced stability and visual fidelity \cite{feng2022impulse, nabizadeh2022covector, deng2023fluid, zhou2024eulerian}. These methods show promise in preserving vorticity and have recently been extended to handle viscous fluid–solid interactions \cite{chen2024solid} and particle-laden flows \cite{li2024particle}. However, they still lack rigorous convergence analysis and benchmarking against established methods, and their flow map formulations for non-conservative forces have yet to be systematically integrated into particle–grid solvers.





%However, there are some concerns with the characteristic mapping method:  (1) It relies on vortex-based formulations, which are not available for velocity-based formulations. Moreover, vortex-based approaches face challenges in recovering the harmonic component of the velocity field, as it does not evolve over time.  (2) The characteristic mapping method is implemented using a complex third-order Hermite interpolation, and it remains unclear whether a simpler construction is possible.  (3) While the current characteristic mapping approach can accurately solve the inviscid Euler equations, it lacks a mechanism for extension to the Navier-Stokes (NS) equations, limiting its applicability.  In this paper, we address each of these issues and propose a new framework—Particle Flow Map (PFM)—which is velocity-based, features a simpler characteristic mapping construction, and is extendable to more general Navier-Stokes equations.

%The velocity field does not naturally conform to a characteristic mapping form, which limits the applicability of characteristic mapping to vortex-based methods. However, since vortex methods do not compute the harmonic component of the velocity field, they face challenges in accurately calculating this component.  (2) The characteristic mapping method is implemented using a complex third-order Hermite interpolation. It remains unclear whether there is a simpler way to construct characteristic mappings.  (3) The current characteristic mapping approach can accurately compute inviscid Euler equations, but it lacks a mechanism to extend it to the Navier-Stokes (NS) equations, making it unsuitable for such computations.  In this paper, we address each of these issues and propose a new framework—Particle Flow Map (PFM)—which is velocity-based, features a simpler characteristic mapping computation, and is extendable to more general Navier-Stokes equations.

==> method.tex <==
\section{Physcial Model}
\begin{table}[h]
    \centering
    \begin{tabular}{|l|p{0.25\textwidth}|p{0.45\textwidth}|}
        \hline
        Notation & Type & Definition\\
        \hline
        $\bm *^f$ & vector/matrix & fluid property\\
        $\bm *^s$ & vector/matrix & solid property\\
        $\bm x$ & vector & particle / mesh vertices location\\
        $\bm *_t$ & scalar/vector/matrix & quantities evaluated at time $t$\\
        $\Phi_{a\to c}$ & vector & Forward flow map from time $a$ to $c$\\
        $\Psi_{c\to a}$ & vector & Backward flow map from time $c$ to $a$\\
        $\mathcal{F}_{a\to c}$ & matrix & Jacobian of forward flow map $\Phi_{a\to c}$\\
        $\mathcal{T}_{c\to a}$ & matrix & Jacobian of backward flow map $\Psi_{c\to a}$\\
        $\bm{u}$ & vector & velocity\\
        $\nabla\bm{u}$ & matrix & velocity gradient\\
        $\bm{m}$ & vector & impulse\\
        $\bm f$ & vector & force\\
        $p$ & scalar & pressure\\
        $\bm \Lambda$ & vector & pressure correction buffer \\
        $\bm \Upsilon$ & vector & external force buffer \\
        $n$ & scalar & reinitialization steps\\
        \hline
    \end{tabular}
    \caption{Notation Table}
    \label{tab:notation_table}
\end{table}

\paragraph{Naming Convension}
We will adhere to the naming conventions in Table~\ref{tab: notation_table}. We will use superscripts to represent the type of a quantity, i.e. $*^f$ for fluid and $*^s$ for solid. We will use subscripts $*_{a}$ to indicate a quantity is evaludated at time $t=a$ and use $*_{a \to c}$ for the evaluation time interval from $a$ to $c$ in flow map notation to represent the duration over which the mapping occurs.

\subsection{Flow Map}
Define a velocity field $\bm u(\bm x, t)$ evaludated at time $t$ and position $\bm x$ where $\forall t \geq 0$ and $\bm x\in\Omega_t$. Within time interval $t=a$ to $t=c$, a fluid parcel $\bm x$ moving with velocity field in such interval from position $\bm x_a \in \Omega_a$ to $\bm x_c \in \Omega_c$ can be associated with a forward flow map $\Phi_{a \to c}:\Omega_a\to\Omega_c$ where $\Omega_a$ and $\Omega_c$ defines the fluid domain at the start and end of the time interval. Similarly, the backward map is defined as $\Psi_{a \to c}: \Omega_c \to \Omega_a$.

To characterize the influence of an infinitisemal change in one domain on another, the Jacobian of the two mapping $\Phi_{a \to c}$ and $\Psi_{c \to a}$ is defined as:
\begin{equation}
    \begin{aligned}
        \mathcal{F}_{a \to c}(\mathbf{x}_a) = \frac{\partial \Phi_{a \to c}(\mathbf{x}_a)}{\partial \mathbf{x}_a}, \\
        \mathcal{T}_{c \to a}(\mathbf{x}_c) = \frac{\partial \Psi_{c \to a}(\mathbf{x}_c)}{\partial \mathbf{x}_c},
    \end{aligned}
    \label{eq:FT}
\end{equation}
respectively and their advection equation defined as
\begin{equation}\label{eq:advection_FT}
    \begin{aligned}
        \frac{D\mathcal{F}_{a\to c}}{Dt}&=\nabla \mathbf{u}(\mathbf{x}) \mathcal{F}_{a\to c},\\
        \frac{D\mathcal{T}_{c\to a}}{Dt}&= -\mathcal{T}_{c\to a}\nabla \mathbf{u}(\mathbf{x}),\\
    \end{aligned}
\end{equation}
which is proved in Appendix~\ref{sec:jacobian_proof} where $\frac{D(\cdot)}{Dt}$ denotes material derivative.

\subsection{Impulse Fluid}
With the four flow map quantities, $\Phi$, $\Psi$, $\mathcal{F}$ and $\mathcal{T}$ and their transport equations, we now have all the essence for an accurate fluid simulation. Following the definition of the impulse form of the Euler equation for invisid fluid, we have:
\begin{equation}
\begin{dcases}
     \frac{D \bm m }{D t} =-\left(\bm \nabla \bm u\right)^T \bm m,\\
    \nabla^2 \varphi = \bm \nabla \cdot \bm m,\\
    \bm u = \bm m - \bm \nabla \varphi,
    \end{dcases}
\label{eq:impulse_euler_eq}
\end{equation}
where $\varphi$ being the gauge freedom depicting the gradient field variation between impulse variable $\bm m$ and divergence free velocity field $\bm u$.
As shown in \citep{}, we can rewrite the transport equation of impulse variable with the four flow map quantities as:
\begin{equation}
\begin{dcases}
    \bm m(x, c)&=\mathcal{T}_{c\to a}^{T}\,\bm{m}(\psi(\bm x),a),\\
    \bm{m}(x, a) &= \mathcal{F}_{a\to c}^T\,\bm m(\phi(\bm x),c).
\end{dcases}
\label{eq:advection_impulse}
\end{equation}

\section{Viscosity \& External Force}
From previous section, we see the transport equations for invisid flow using impulse variables. Below, we extend such form to incorporate vicosity and external forces and derive the transport equation using flow map under such condition.
\subsection{Continuous Form}
Define $\bm q =\bm m - \bm u$, we can rewrite Eq.~\ref{eq:impulse_euler_eq} as:
\begin{equation}
    \begin{dcases}
        \frac{D \bm u}{Dt} = -\nabla p + \bm f,\\
        \frac{D\bm m}{Dt}=-(\nabla \bm u)^T \bm m\\
        \bm u = \bm m - \bm q.\\
    \end{dcases}
    \label{eq:sfi_u}
\end{equation}
where $\bm f$ includes viscosity $\nabla^2 \bm u$ under divergence free velocity field and external forces like gravity. Due to the presence of external forces, the expression for gauge variable $\bm q$ need to be rederived. Notice without the presence of external forces, $\bm q = \nabla \varphi$ for $q$ only needed to include pressure. 

Using vector identity $\nabla (\frac{1}{2} |\bm u|^2) = (\nabla \bm u)^T \bm u$ and Eq.~\ref{eq:sfi_u}, we have:
\begin{equation}
    \begin{split}
        &\frac{D\bm u}{Dt} = \frac{D \bm m}{D t} - \frac{D \bm q}{D t},\\
        &-\nabla p + \bm f + \frac{D \bm q}{D t} + (\nabla \bm u)^T(\bm u + \bm q) = 0,\\
        &\frac{D \bm q}{D t} + (\nabla \bm u)^T\bm q + \nabla(\frac{1}{2}|\bm u|^2) - \nabla p + \bm f = 0,\\
    \end{split}
\end{equation}
By applying Eq.~\ref{eq:advection_FT} and flow map identity $\mathcal{F}\mathcal{T} = \mathcal{I}$, we have:
\begin{equation}
    \begin{split}
        &\frac{D \bm q}{D t} + \mathcal{T}^T \frac{D \mathcal{F}^T}{D t}\bm q + [\nabla(\frac{1}{2}|\bm u|^2) - \nabla p + \bm f] = 0,\\
        &\frac{\mathcal{F}^T D\bm q}{D t} + \frac{D \mathcal{F}^T}{D t}\bm q + \mathcal{F}^T[\nabla(\frac{1}{2}|\bm u|^2) - \nabla p + \bm f] = 0,\\
        &\frac{D\mathcal{F}^T\bm q}{D t} = \mathcal{F}^T[\nabla p - \nabla(\frac{1}{2}|\bm u|^2)]  - \mathcal{F}^T\bm f.
    \end{split}
    \label{eq:buffer_continue}
\end{equation}
Assuming we have the mapping time interval between $t=a$ to $t=c$, by integrating both sides within such time interval, we derive:
\begin{equation}
    \begin{split}
        \mathcal{F}_{a \to c}^T\bm q_c = \int_a^c \mathcal{F}^T_{a \to \tau} (\nabla p_{\tau} - \nabla\frac{1}{2}\bm |u_{\tau}|^2)d\tau -\int_a^c \mathcal{F}^T_{a\to \tau}\bm f_{\tau} d\tau, \\
        \bm q_c = \mathcal{T}_{c\to a}^T[\int_a^c \mathcal{F}^T_{a \to \tau} (\nabla p_{\tau} - \nabla\frac{1}{2}\bm |u_{\tau}|^2)d\tau -\int_a^c \mathcal{F}^T_{a\to\tau}\bm f_{\tau} d\tau].
    \end{split}
    \label{eq:buffer_continue}
\end{equation}
With the expression for $\bm q$ at time $c$, we give the expression for impulse form for the general Navie-Stoke equation as:
\begin{equation}
    \begin{dcases}
        \bm m_c = \mathcal{T}_{c\to a}^{T}\,\bm{m}_a,\\
        \bm q_c = \mathcal{T}_{c\to a}^T[\int_a^c \mathcal{F}^T_{a \to \tau} (\nabla p_{\tau} - \nabla\frac{1}{2}\bm |u_{\tau}|^2)d\tau -\int_a^c \mathcal{F}^T_{a\to\tau}\bm f_{\tau} d\tau].\\
        \bm u_c = \bm m_c - \bm q_c
    \end{dcases}
    \label{eq:sfi_u_continuous}
\end{equation}
where $\tau$ represents time instance within the mapping interval and $\bm f$ notes external forces and viscous force.

\section{Particle Flow Map}
Observing that Eq.~\ref{eq:sfi_u_continuous} can be written with a Lagrangian path integral form and noticing that using particle representation with Eq.~\ref{eq:advection_FT} perfectly sastifies flow map identity $\mathcal{F}\mathcal{T}=\mathcal{I}$ as shown below, we propose to use Lagrangian particles for discritizing the above equation.
\subsection{Geometric Representation}
Particles naturally represent flow maps. As illustrated in Figure~\ref{fig:pfm}, consider a particle that moves according to a spatiotemporal velocity field $\bm u(\bm x,t)$. The trajectory of this particle, which begins at time $a$ and concludes at time $c$, defines both the forward map $\Phi_{a \to c}$ and the backward map $\Psi_{c\to a}$. Quantities such as $\mathcal{F}$ and $\mathcal{T}$, which are obtained through path integrals along the particle's trajectory (as demonstrated in Equation~\ref{eq:advection_FT} for calculating $\mathcal{F}$ and $\mathcal{T}$), can be computed by performing integrals while tracking the particle's movement along its path.

We will next show that a particle representation serves as a perfect flow map, i.e. perfectly sastifies the identities (See proof in Appendix~\ref{sec:perfect_flow_map})
\begin{equation}
    \begin{dcases}
        \bm x_a =\bm \Psi_{c\to a}\circ\bm \Phi_{a\to c}(\bm x_a), \\
        \bm x_c = \bm \Phi_{a\to c} \circ\bm \Psi_{c\to a}(\bm x_c).
    \end{dcases}
    \label{eq:roundtrip_psi}
\end{equation}
and 
\begin{equation}
    \begin{dcases}
        \bm I = \mathcal{F}_{a\to c} (\bm x_a)\mathcal{T}_{c\to a}(\bm x_c),\\
        \bm I = \mathcal{T}_{c\to a}(\bm x_c)\mathcal{F}_{a \to c}(\bm a).
    \end{dcases}
    \label{eq:roundtrip_T}
\end{equation}

Consider a particle that moves according to a flow map $\Phi_{a \to c} (\bm x_a)$, starting from point $\bm x_a$ at time $a$ and arriving at point $\bm x_c$ at time $c$. If we reverse this motion and allow the particle to move from $\bm x_c$ at time $c$ back to the starting point using the backward flow map $\Psi_{c\to a}(\bm x_c)$, the particle will trace the same path in reverse order. Therefore, particle representation inheritly satifies Eq.~\ref{eq:roundtrip_psi}

Next, we will establish that a particle flow map aligns with Eq.~\ref{eq:roundtrip_T}. We conducted a numerical experiment for this purpose: As illustrated in Figure~\ref{fig:motivational_experiment}(a) and (b), we calculated $\mathcal{F}\mathcal{T}$ for particles moving within a steady velocity field defined by $\omega(r) = -0.01(1 - e^{-r^2/0.02^2})/r$ and $u(x, y, r) = \omega(r)\begin{bmatrix}-y\\ x\end{bmatrix}$, where $x$ and $y$ represent point locations and $r$ indicates the distance from the point to the rotation center at $(0.5, 0.5)$. As shown in Figure~\ref{fig:motivational_experiment}(c), we observed that $\mathcal{F}\mathcal{T}$ closely approximates the identity, with errors on the order of $10^{-6}$ across 200 steps. These results affirm that particle represnetation comply with  Eq.~\ref{eq:roundtrip_T}.

\subsection{Discretized Advection Equations}
As shown above, particle representation is perfectly suitable for discritizing flow map applications for its natrual support on path integration and satisfaction for flow map identities. Therefore, we carry physical quantities $\bm m$, $\Phi$, $\Psi$, $\mathcal{T}$ and $\mathcal{F}$ on particles and direct them with their advection equations, i.e. Eq.~\ref{eq:advection_FT} and Eq.~\ref{eq:advection_impulse}. 

To aid the calculation of Eq.~\ref{eq:buffer_continue}, we define the two discretized integral for $\bm q$ as two particle buffers namely pressure correction buffer $\bm \Lambda$ and external force buffer $\bm \Upsilon$:
\begin{equation}
    \begin{dcases}
        \bm \Lambda_c &= \int_a^{c} \mathcal{F}^T_{a \to \tau} \nabla (p_{\tau} - \frac{1}{2}|\bm{u_{\tau}}|^2)d\tau,\\
        \bm \Upsilon_c &= \int_a^{c} \mathcal{F}^T_{\tau\to a} \bm f_{\tau} d\tau.
    \end{dcases}
    \label{eq:external_force}
\end{equation}
where $p$ is the pressure from Poisson projection from previous step. To reform such integral into single step advection equations for the two buffers, we assume current time step as $t=c$ and previous time step $t-\Delta t$ as $t=b$ and single step update is from $t=b$ to $t=c$. In the definition of $\bm m$, it is important to note that $\bm u$ is a divergence-free velocity field. Consequently, Equation~\ref{eq:sfi_u_continuous} includes pressure at time $c$, which is unknown and needs to be resolved through Poisson projection. Similarly, the term $\frac{1}{2}\bm u_c^2$ remains unknown and requires resolution. Therefore, the actual divergent velocity field $u_c^*$ at time $c$ must remove the pressure component from Equation~\ref{eq:sfi_u_continuous}, and we approximate the original expression for $\frac{1}{2}\bm u_c^2$ using $\frac{1}{2}\bm u_b^2$. In practice, we utilize $\frac{1}{2}\bm u_{\text{mid}}^2$ as a result of our implementation of mid-point velocity approximation. Hence, the advection equation for $\bm \Lambda$ and $\bm \Upsilon$ are given as:
\begin{equation}
\begin{split}
        \bm \Lambda_c &= \bm \Lambda_b + \mathcal{F}^T_{[a\to c]}\Delta t(\nabla p_c - \nabla\frac{1}{2}|\bm u_c|^2)\\
        \bm \Upsilon_c &= \bm \Upsilon_b + \mathcal{F}^T_{[a\to c]}\Delta t\bm f_c
\end{split}
\end{equation}
and the expression for the divergent $\bm u_c^*$ becomes:
\begin{equation}
    \begin{aligned}
        \bm u_c^* = \mathcal{T}_{c\to a}^T(\bm m_a) -\mathcal{T}_{c\to a}^T(\mathcal{F}_{a\to b}^T\bm q_b) +\Delta t \bm f_c + \Delta t(\nabla\frac{1}{2}|\bm u_b|^2)
    \end{aligned}
\end{equation}
With all update equations in hand, the advection equations for the whole system can be written as:
\begin{equation}
    \begin{dcases}
        \bm m_c = \mathcal{T}_{c\to a}^T\bm m_a,\\
        \bm u_c^* = \bm{m}_c - \mathcal{T}_{c\to a}^T (\bm \Lambda_b - \Upsilon_b) + \nabla \frac{1}{2}|\bm{u_b}|^2 \Delta t + \bm f_c\Delta t,\\
        \nabla^2 p_c = \frac{1}{\Delta t}\nabla \cdot \bm u_c^*\\
        \bm u_c = \bm u_c^* - \Delta t \nabla p_c\\
        \bm \Lambda_c = \bm \Lambda_b + \mathcal{F}^T_{a\to c}\Delta t(\nabla p_c - \nabla\frac{1}{2}|\bm u_c|^2),\\
        \bm \Upsilon_c = \bm \Upsilon_b + \mathcal{F}^T_{a\to c}\Delta t\bm f_c.
    \end{dcases}
    \label{eq:update_equation}
\end{equation}

\section{Time Integration with Eulerian Lagrangian Framework}
In order to simulate incompressible flow, we choose to adapt an Eulerian-Lagrangian framework. Specifically, physical quantities are accurately transported using Lagrangian particles with their advection equations outlined in Eq.~\ref{eq:update_equation} and the incompressibiliy constraint is enforced on the Eulerian mesh. The communication between the two representations are conducted with a Particle-to-Grid (P2G) and Grid-to-Particle (G2P) process. Below, we specify the calculation of each quantity.

\subsection{Flow Map Calculation} Flow maps are carried directly on particles. Since both the forward and backward particle flow maps coincide along the same particle path, we directly apply Equation~\ref{eq:advection_FT} for advection of $\mathcal{T}$ and $\mathcal{F}$. As flow map is a geometric concept, it's Jacobian $\mathcal{F}$ and $\mathcal{T}$ quickly get distorted under turbulant flow field especially when flow map range get overly enlonged. Following common practice in \citep{}, we perform reinitialization every $n$ step where time $a$ is reset to time $c$ as the new starting point and flow map Jacobian is set to identity:
\begin{equation}
    \mathcal{F}_{a \to c} \gets \mathcal{I}, \text{ } \mathcal{T}_{c \to a} \gets \mathcal{I}.
\end{equation}

\subsection{Calculation of $\bm m_c$} Impulse variable is carried on particle. By applying the first equation in Eq.~\ref{eq:update_equation} after the advection of flow map at each step, we can obtain the accurate impulse variable advected through flow map. The reinitialization of impulse variable happens with the reset of flow map Jacobian by ecalibrateing it using the interpolated the velocity field at time c:
\begin{equation}
    \label{eq:reinit_imp_long}
    \bm m_{a}^p \gets \sum_i w_{ip} \bm u_i \,/\, \sum_i w_{ip}.
\end{equation}
Here, $w_{ip}$ is the interpolation weight used in \citep{} and $\bm u_i$ is the divergence free velocity field solved on grid at time $c$.

\subsection{Calculation of $\bm u_c^*$} $u_c^*$ is first calculated on particles and then transferred to grid using a P2G procedure. Suppose we have the two buffer $\bm \Lambda_b$ and $\bm \Upsilon_b$ from previous step, the calculation of  divergent velocity $\bm u_c^*$ directly follows the second equation in Eq.~\ref{eq:update_equation}. By using midpoint advection scheme, we calculate $\nabla \frac{1}{2}\bm u_{\text{mid}}^2$ on particles through interpolation on grid where G2P is performed with typical APIC\citep{} kernel. $\bm f_c$ includes viscosity and gravity.  For gravity, it's natually stored and on particles. For viscosity, it's calculated following:
\begin{equation}
    \bm f_{c}^p \gets \sum_i \nabla \bm u_i^T \nabla w_{ip} \,/\, \sum_i w_{ip}.
\end{equation}
where $\nabla \bm u$ on grid is obtained through first performing G2P with 
\begin{equation}
    \nabla \bm u_{c}^p \gets \sum_i \bm u_i \nabla w_{ip} \,/\, \sum_i w_{ip}.
\end{equation}
and then performing P2G with
\begin{equation}
    \nabla \bm u_i \gets \sum_p w_{ip} \nabla \bm u_c^p \,/\, \sum_p w_{ip}.
\end{equation}
Now, all quantities are on particles, together with $\bm \Lambda$ and $\bm \Upsilon$ calculated from the previous frame, we get $\bm u_c^*$ following Eq.~\ref{eq:update_equation}. After this, $\bm u_c^*$ is transferred to grid with 
\begin{equation}
    {\bm {u_c^*}}_{i} \gets \sum_p w_{ip} {\bm {u_c^*}}^p \,/\, \sum_p w_{ip}.
\end{equation}
Here, we use upperscript $p$ for particle and subscript $i$ for grid.

\subsection{Poisson Projection for Calulation of $p_c$ and $\bm u_c$} Poisson equation is solved with the typical MGPCG solver and the divergent part is corrected using the pressure gradient. After retriving the divergence free velocity field $\bm u_c$ following the third and forth equation in Eq.~\ref{eq:update_equation}, we transfer $p$ from grid to particle using:
\begin{equation}
    p_{c}^p \gets \sum_i \bm p_i w_{ip} \,/\, \sum_p w_{ip}.
\end{equation}


\subsection{Calculation of $\bm \Lambda_c$ and $\bm \Upsilon_c$} $\bm \Lambda_c$ and $\bm \Upsilon_c$ are stored on particle. To calculate $\bm \Lambda_c$, we follow the update equation provided in Eq.~\ref{eq:update_equation}. After resolving the Poisson projection for time step $c$, we obtain ${p_c}$ and $\bm u_c$ on the grid. Subsequently, we compute $\nabla (p_{c} - \frac{1}{2}|\bm{u_{c}}|^2)$ on the grid and transfer this value to the particles through a G2P process. This value is then accumulated on $\bm \Lambda_c$ by mapping it back to the initial frame $a$ using $\mathcal{F}_{a \to c}$. The gradient operator is computed as the gradient of the weight kernel similar to the calculation of viscosity in above. With $\mathcal{F}_{a\to c}$ and $\bm f_c$ already calculated in previous procedures within current timestep, we directly apply the last equation in Eq.~\ref{eq:update_equation} and add it to $\bm \Upsilon_b$. Reinitialization of the two buffer happens at the same time with flow map reinitialization by setting the value of the two buffers to 0 on each particle.

\subsection{Midpoint Integration}
We utilize a leapfrog-style energy preservation temporal integration scheme to enhance vorticity preservation. Such choice is commonly used for applications require enegy preservation. At time $c$, we advect fluid velocity $\bm u_b$ by half timestep without using flow map and solve Poisson equation to get $\bm u^{\text{mid}}_c$. Such velocity is then used for advection of $\mathcal{F}_{a \to c}$ and $\mathcal{T}_{c \to a}$ and for calculation of the term $\nabla \frac{1}{2}|\bm u|^2$ in $\bm u_c^*$.

\subsection{CFL Condition}
We compute $\Delta t$ with velocity field $\bm{u}_i$, the CFL number and grid resoltuion $\Delta x$ by
\begin{equation}
    \Delta t = \frac{C\Delta x}{max(\bm u)}
\end{equation}

\subsection{Time Integration}


==> notes.tex <==
4/29/2025
1. 多行公式都加个大括号 Done
2. 公式的逗号句号标点都要注意 Done
3. 3.1里的X和x和我们习惯的用法不一样？能不能不要用Y，而是只用X，x？(这个要不算了，小x zhiqi用来定义别的东西了，不好改)
4. 加一个notation table (Done)




==========================================================

introduction

- impulse gauge变量被作为一种Lagrangian粒子方法在xxx文章中被提出，讲一下背景
- 传统impulse粒子方法有一些固有问题，比如impulse在演化过程中会不断变大，导致数值不稳定（另外还有什么弱点也想一下）
- 在最近的几年里，CG领域提出了把impulse变量带在粒子上，作为一种粒子网格法来发展，这种方法被结合进了flow map观点和APIC的gradient插值两种技术，展示了很好的保涡能力。但这种方法作为一种图形学中focus在涡旋结构保持的视觉效果的算法，它的物理精确性没有得到严格验证。另外，作为一种Navier Stokes solver，它处理非保守力的flow map方法也没有严格的集成到粒子-网格solver中。
- 本文提出了一种基于PFM的NS solver，完整的建立了在粒子-网格基础上的impulse gauge solver







experiments

For pure convergence tests for flow map:
convergence test for mapping
energy conservation for single and taylor green vortex
other tests with analytical solution having vortices
flow map + impulse + viscosity
2D RT不稳定实验
2D卡门涡街
3D ink在不同re的表现
For two phase fluid with surfrace 
bubble shape changing experiment (yuchen之前给我看过他做过)
2D 在不同的parameter下，小球入缸产生difference capillary wave
yuchen的涡在水底对水面影响的那个实验 + 真实数据截图
其他的asia里面的实验
two-way coupling
鱼游泳速度跟收缩parameter的关系的图表
school of fish的例子
IBM的各种例子（可以把上周的火放上？）
加几个passive下落的3D mpm例子
sediment flow
ink drop跟物理期刊的一些对比
我们设计的一些实验画成图表比如reinit频率跟分叉的关系等


==> related_work.tex <==
\section{Related Work}
%  characteristic mapping
\subsection{characteristic mapping}
A characteristic map (flow map) method is commonly regarded as a geometric approach for advecting arbitrary sets \cite{kohno2013new,mercier2020characteristic}. In \cite{yin2021characteristic}, this approach was extended to transport flow quantities stemming from the semi-Lagrangian gradient augmented level set method \cite{nave2010gradient} and the jet scheme \cite{seibold2011jet}, thereby fully exploiting the characteristic structure of two-dimensional fluid flow. In this framework, advected fluid quantities are constructed as the composition of the initial condition with the characteristic map. This formulation permits the reconstruction of vorticity via the pullback of the initial condition by the characteristic map, enabling arbitrarily fine spatial resolution due to the functional definition of the solution. In \cite{yin2023characteristic}, the method was further extended to the three-dimensional incompressible Euler equations in vorticity form. This extension addresses the stretching term in vorticity advection, avoiding the rapid growth of both vorticity magnitude and its gradient \cite{fefferman2006existence} by incorporating the Jacobian of the characteristic map into the computation of the vorticity, thereby enhancing the method's regularization. 
%  impulse&vortex方法
\subsection{Vortex \& Impulse methods}
Advected quantities in fluid dynamics can be categorized by their differential forms-0-form, 1-form, and 2-form—which correspond respectively to point elements, surface elements, and line elements \cite{wu2007vorticity}. Typical examples include velocity, impulse, and vorticity. While the vorticity formulation of the Navier–Stokes equations has been extensively studied (see, e.g., \cite{mimeau2021review} for a recent survey), the impulse formulation has attracted relatively little attention. The impulse variable, introduced by Buttke \cite{buttke1992lagrangian}, offers an alternative description of the incompressible Navier–Stokes equations by incorporating a gauge variable and an associated gauge transformation \cite{oseledets1989new, roberts1972hamiltonian, buttke1993velicity}. Subsequent studies have explored various aspects of gauge freedom, including its application to surface turbulence \cite{buttke1993velicity, buttke1993turbulence}, its influence on numerical stability \cite{weinan2003gauge}, and its role in fluid-structure interactions \cite{cortez1996impulse, summers2000representation}. More recent work by Saye et al. \cite{saye2016interfacial, saye2017implicit} has exploited gauge freedom to address interfacial discontinuities in density and viscosity in free-surface flows and fluid–structure coupling.

In this work, we derive the functional for an impulse formulation of the incompressible Navier–Stokes equations by leveraging the geometric nature of fluid flow through the use of a flow map. We present our approach as a hybrid Eulerian-Lagrangian method. Our formulation is in parallel to PIC/FLIP \cite{brackbill1986flip, edwards2012high} and APIC \cite{jiang2017angular, ding2020affine} methods used for velocity advection and vortex-in-cell methods \cite{christiansen1973numerical, couet1981simulation, cottet2004advances, rossinelli2010gpu} for vorticity advection, offering a robust alternative that enhances vorticity preservation with numerical accuracy while mitigating numerical instabilities.
%  粒子网格法
\subsection{Eulerian–Lagrangian Methods} Eulerian–Lagrangian approaches employ a grid-based framework for computing pressure and viscous terms, while Lagrangian particles handle advection to reduce numerical diffusion. The Particle-in-Cell (PIC) framework introduced by \cite{harlow1964particle} initially suffered from smoothing errors in particle-to-grid transfers. Fluid-Implicit-Particle (FLIP) \cite{brackbill1986flip} overcame this issue by updating particle velocities according to velocity increments, preserving vorticity more effectively. Subsequent advancements introduced higher-order moment transfers in methods like APIC \cite{jiang2017angular}, XPIC \cite{hammerquist2017new}, and EPIC \cite{frey2022epic}, culminating in HOPIC \cite{edwards2012high}, which leverages Moving Least Squares (MLS), Weighted Essentially Non-Oscillatory (WENO) schemes, and Runge–Kutta integration to achieve fifth-order accuracy. While these methods effectively minimize dissipation, their complex interpolation kernels can lead to increased computational expense. To mitigate this, polynomial expansions (PolyPIC) \cite{fu2017polynomial} and unified MLS-based frameworks \cite{hu2018moving} have been devised, offering improved accuracy at more manageable costs.
%  图形学方法
\subsection{Graphics Methods}
In computer graphics, alternative fluid formulations have also gained traction for enhanced stability and visual fidelity. Impulse-based approaches, for instance, reparameterize momentum to handle incompressibility \cite{feng2022impulse}, while vortex-focused methods represent fluid flow in terms of vorticity \cite{park2005vortex, selle2005vortex, zhang2014pppm, xiong2021incompressible}, thereby naturally preserving circulation. Another research direction aims to reduce numerical diffusion using flow map-based techniques, first introduced to the graphics community by \cite{tessendorf2011characteristic}. Recent advancements have explored bidirectional flow maps \cite{qu2019efficient} and combined impulse-based models with flow map representations \cite{nabizadeh2022covector}. Neural Flow Maps (NFM) \cite{deng2023fluid} integrate impulse formulations with neural network-based velocity compression, enabling high-precision reconstruction of flow maps. NFM has also been extended to vortex simulations \cite{wang2024eulerian}, blending vorticity preservation with flow map advection. Meanwhile, Particle Flow Maps (PFM) \cite{zhou2024eulerian} combine an impulse-based solver on a grid with Lagrangian particle tracking, showing promise for vorticity retention and recently adapted to viscous fluid–solid interactions \cite{chen2024solid} and laden flows \cite{li2024particle}. However, these methods lack rigorous convergence tests and benchmarking against established schemes.
